Bridging the Domain Gap for Ground-to-Aerial Image Matching

The visual entities in cross-view images exhibit drastic domain changes due to the difference in viewpoints each set of images is captured from. Existing state-of-the-art methods address the problem by learning view-invariant descriptors for the images. We propose a novel method for solving this task by exploiting the generative powers of conditional GANs to synthesize an aerial representation of a ground level panorama and use it to minimize the domain gap between the two views. The synthesized image being from the same view as the target image helps the network to preserve important cues in aerial images following our Joint Feature Learning approach. Our Feature Fusion method combines the complementary features from a synthesized aerial image with the corresponding ground features to obtain a robust query representation. In addition, multi-scale feature aggregation preserves image representations at different feature scales useful for solving this complex task. Experimental results show that our proposed approach performs significantly better than the state-of-the-art methods on the challenging CVUSA dataset in terms of top-1 and top-1% retrieval accuracies. Furthermore, to evaluate the generalization of our method on urban landscapes, we collected a new cross-view localization dataset with geo-reference information.

==> sections/method.tex <==
% \clearpage
\section{Method}
% The proposed 
%We provide an overview of cross-view synthesis GAN, briefly discuss about the loss function used in image retrieval networks and then explain our proposed method \MS{it should not one method, not several method, do not use plural} in this section. 



% ----------------------------------------------------------------------------



% \subsection{Conditional GAN for Cross-View Synthesis} 
% In this work, we synthesize the aerial images from ground-level panorama to use them for image matching. Previous works \cite{Regmi_2018_CVPR, regmi2018cross, Deng:2018:LDG:3274895.3274969, 8490997} have been successful in image translation between aerial and ground-level cropped (single camera) images. Zhai \textit{et al.} \cite{zhai2017crossview} explored the possibility of synthesizing ground-level panorama from aerial images. Here, we transform the query ground level panorama to aerial view. 

% We adopt X-Fork generator architecture  of \cite{Regmi_2018_CVPR} to train the GAN. The X-Fork is a multi-task learning architecture that synthesizes cross-view image as well as semantic segmentation map. Learning to synthesize segmentation map as an auxiliary task greatly helps cross-view synthesis by enforcing the network to preserve the semantic consistency in the target image. 

% The generator of X-Fork has an encoder and two decoders. The network consists of blocks of Convolution, Batch Normalization and Leaky ReLU layers. Convolutional kernels of size 4 x 4 with a stride of 2 are used that downsamples features after each convolution. Since our input is panorama which is of rectangular size, we reshape the features at the bottleneck into square (2 x 2), and then apply multiple upconvolution operations to generate 512 x 512 resolution target image. The six blocks of decoders share the weights whereas the final two blocks don't. One of the branches learns weights to synthesize the target view image while the other branch generates the corresponding semantic map. We first train the GAN to generate the cross-view image $I_a'$ for the ground panorama $I_g$. Next, we use the synthesized images for joint feature learning in our proposed methods.


%\subsection{Conditional GAN for Cross-View Synthesis} 

In this work, we synthesize the aerial images from ground-level panorama to use them for image matching. 
%Previous works \cite{Regmi_2018_CVPR, regmi2018cross, Deng:2018:LDG:3274895.3274969, 8490997} have been successful in image translation between aerial and ground-level cropped (single camera) images. Zhai \textit{et al.} \cite{zhai2017crossview} explored the possibility of synthesizing ground-level panorama from aerial images. Here, we transform the query ground level panorama to aerial view. 
We adopt X-Fork generator architecture  of \cite{Regmi_2018_CVPR} to train the GAN. 
%The X-Fork is a multi-task learning architecture that synthesizes cross-view image as well as semantic segmentation map. Learning to synthesize segmentation map as an auxiliary task greatly helps cross-view synthesis by enforcing the network to preserve the semantic consistency in the target image. 

%We make the following modifications to the X-Fork architecture. Since our input is panorama (rectangular in shape), the feature maps at the bottleneck are also rectangular (1x4). 
 %We reshape the features into squares (2 x 2), and then apply multiple upconvolution operations to generate 512 x 512 resolution aerial images. Next, we exploit the object edges in input images to provide the network with notion of object shapes and boundaries.  We employ Canny Edge Detection \cite{canny1987computational} to obtain the edgemaps of the inputs.  We stack an edgemap together with the panorama, along the channels to create a 4-channel input; 3 RGB-channels and 1 edgemap channel. 
%  We observe that the 
 %The detailed architecture of modified X-Fork network is provided in the supplementary.

% ----------------------------------------------------------------------------



%\subsection{Weighted Soft-margin Triplet Loss}
% Given the success of soft-margin triplet loss in previous works \cite{DBLP:journals/corr/HermansBL17, Vo2016} and its weighted version in \cite{Hu_2018_CVPR} for image retrieval tasks, we also use the same loss function in our training. 

Consider a feature embedding $f_{g}$ for ground-level image, $f_{a-pos}$ for the corresponding matching aerial image and a non-matching aerial image feature $f_{a-neg}$.  The triplet loss \cite{DBLP:journals/corr/HermansBL17} aims to pull the matching feature $f_{a-pos}$ closer to $f_{g}$ while at the same time push $f_{a-neg}$ away. Here, if $d_{p}$ is the Euclidean distance between positive samples ($f_{g}$, $f_{a-pos}$) and $d_{n}$ is the Euclidean distance between negative/non-matching samples ($f_{g}$, $f_{a-neg}$), we try to minimize $d_{p}$ as well as maximize $d_{n}$ using triplet loss. The triplet loss is as shown below:


\vspace{-15pt}
\begin{equation}\label{triplet} 
L_{triplet} = max( 0, m + d_{p} - d_{n}),
\end{equation}

\noindent where, $m$ is a margin that specifies a minimum distance between non-matching pairs. 

In order to avoid the necessity of explicitly deciding the margin for triplet loss, soft-margin triplet loss is popular and is expressed as shown in Equation \ref{triplet-soft}.

\vspace{-15pt}
\begin{equation}\label{triplet-soft}
 L_{soft} = ln( 1 + e^d),
\end{equation}

\noindent where d = $d_{p}$ - $d_{n}$.

We use the weighted soft margin triplet loss\cite{Hu_2018_CVPR} as shown in Equation \ref{weighted-soft}. We use  $ \alpha $ = 10, which  results in better convergence than $ \alpha $ = 1.

\vspace{-15pt}
\begin{equation}\label{weighted-soft}
 L_{weighted} = ln( 1 + e^{\alpha d}).
\end{equation}

 
% ----------------------------------------------------------------------------


\begin{figure}[t]
\begin{center}
  \vspace{-10pt}
   \includegraphics[width=0.98\linewidth]{images/two-stream.pdf}
\end{center}
   \caption{\small Two stream architecture with multi-scale feature aggregation. $\oplus$ represents channelwise concatenation of feature maps.}
\label{fig:two-stream}
   \vspace{-5pt}
\end{figure}
% ----------------------------------------------------------------------------


\subsection{Two Stream Network} 
We employ Siamese-type architecture,  as shown in Figure \ref{fig:two-stream}, where the two encoders do not share the weights. Since the cross-view images are captured from very different viewpoints, entities in one view look different than the entities in the other view. The two branches operate on these sets of diverse images, so it is understandable that the weight sharing is not a good choice. 
Next, we employ multi-scale feature aggregation by preserving the features at three scales. We elegantly exploit the inherent multi-scale pyramidal structure of features at multiple layers of deep neural networks. We consider the features from final three convolutional layers, conv\_6, conv\_7 and conv\_8 layers. These features are aggregated and followed by a fully connected layer to obtain the representation for images in each view. 



Let $X_i$ be a feature map at  \textit{i}$^{th}$ convolutional layer, with feature dimension  $C_i$ x $H_i$ x $W_i$,  where $C_i$, $H_i$ and $W_i$ are channels, height and width respectively. We flatten the feature maps before concatenating them along the channels to obtain the aggregated feature of size: ($C_6$ * $H_6$ * $W_6$) + ($C_7$ * $H_7$ * $W_7$) + ($C_8$ * $H_8$ * $W_8$). Final layer is a fully connected layer that reduces the feature dimensions to 1000. 

We conduct experiments with image pairs of ($I_g$, $I_a$) and ($I_a'$, $I_a$) using two-stream network as baselines in our work. Here, $I_g$ is the ground query image, $I_a$ is the aerial image from reference database and $I_a'$ is the synthesized aerial image generated from $I_g$. We use weighted soft-margin triplet loss shown in Equation \ref{weighted-soft} to learn the feature representations for the image pairs.


% ----------------------------------------------------------------------------

\begin{figure}
\begin{tabular}{c}
\subcaptionbox{Joint Feature Learning: Jointly training on $I_g$ and $I_a'$ through matching them against $I_a$ employing auxiliary loss between $f_a'$ and $f_a$ helps to pull features $f_g$ and $f_a$ closer, and minimize the domain gap between two features when trained using two-stream network shown in Figure \ref{fig:two-stream}.  
\label{fig:aux-loss}} {\includegraphics[width=0.95\linewidth]{images/auxGAN_II.pdf}}\\ \\
\subcaptionbox{Feature Fusion. We fuse the features $f_g$ and $f_a'$ obtained from \ref{fig:aux-loss} and find their common representation $f^*_g$ using fully-connected layer. Similarly, $f_a$ is mapped to $f^*_a$, a domain closer to $f^*_g$. The fully-connected layers are trained, whereas the rest of the network is frozen. \label{fig:fusion-net}} {\includegraphics[width=0.95\linewidth]{images/auxGAN_with_fusion.pdf}}

\end{tabular}
% \vspace{-10pt}
\caption{\small Architectures for our proposed approaches. The green and blue triangles are encoders with the same architecture as encoder branches shown in Figure \ref{fig:two-stream}.}
 \vspace{-10pt}
\end{figure}



% ----------------------------------------------------------------------------


\subsection{Joint Feature Learning and Fusion} 
In this work, we utilize synthesized images constructively as complementary information for the network to exploit during joint feature learning. 
We build upon the generative power of conditional GANs to generate the aerial image for query ground-level panorama. 
Ideally, the synthesized aerial image should be sufficient and capable to retrieve its matching gallery image to justify that cross-view image matching can be solved as cross-view image synthesis followed by the same-view matching. 
% the same-view matching is easier than cross-view matching. 
But, the cross-view synthesis has its own challenges as explained in \cite{Regmi_2018_CVPR} and the synthesized images are noisy; hence cannot be relied upon wholly. Therefore, we attempt to use the synthesized image $I_a'$, as a complementary information during training to bring features $f_g$ and $f_a$ closer by adding an auxiliary loss.  
Next, we fuse the features $f_g$ and $f_a'$ to obtain a joint feature representation $f^*_g$ of query image, and compare it against the aerial feature representation $f^*_a$. 
We combine the features  $f_a'$ and $f_g$ since we expect them to have complementary features, which will be helpful in image retrieval. We provide further explanation below:  


% ----------------------------------------------------------------------------


% \subsubsection{Constructive Learning with Auxiliary Loss} 
\subsubsection{Joint Feature Learning with Auxiliary Loss} 
% \hspace{10pt} In this work, we utilize synthesized images constructively as complementary information for the network to exploit during joint feature learning. 
% We build upon the generative power of conditional GANs to generate the aerial image for query ground-level panorama. 
% Ideally, the synthesized aerial image should be sufficient and capable to retrieve its matching gallery image to justify the same-view matching is easier than cross-view matching. But, the cross-view synthesis has its own challenges as explained in \cite{Regmi_2018_CVPR} and the synthesized images are noisy; hence cannot be relied upon wholly. So, we attempt to use the synthesized image $I_a'$, as a complementary information during training to bring features $f_g$ and $f_a$ closer by adding an auxiliary loss.  
\hspace{10pt} We present a novel approach to leverage the synthesized aerial image in feature learning to assist during cross-view image retrieval.
We employ joint feature learning for real ground query image, ($I_g$), and its transformed version, ($I_a'$). 
The features, $f_g$ for $I_g$ and $f_a'$ for $I_a'$ are jointly optimized against the features $f_a$ for $I_a$. 
The encoder branches for $I_a'$ and $I_a$ share the weights, since both images represent aerial domain. 
This way, the aerial encoder learn weights suitable for the synthesized image $I_a'$ as well as the real image $I_a$. 
Thus, $f_a'$ effectively forces the features $f_a$ to be closer to $f_g$ and bridges the domain gap between the two views. 
This is possible because the transformed image $I_a'$  captures representations of $I_g$ which are easier for the network to learn from $I_a'$ than it would be when comparing $I_a$ directly against $I_g$. 


The network architecture for joint feature learning is shown in Figure \ref{fig:aux-loss}. The encoder blocks are shown in green (for ground image) and blue (for aerial image) triangles. Each encoder consists of the same layers as a branch in Figure \ref{fig:two-stream}. We train our network jointly on these three sets of images ($I_g$, $I_a'$ and $I_a$) using Equation \ref{joint-loss}.  Here, $\lambda_1$ and $\lambda_2$ are balancing factors between the losses for ($I_g$, $I_a$) and ($I_a'$, $I_a$) pairs respectively. During the testing, only the encoders for $I_g$ and $I_a$ are used for feature extraction of real ground and aerial images and retrieval is conducted between the ground image features $f_g$ and aerial image features $f_a$.
% to perform cross-view matching. 

\vspace{-10pt}
\begin{equation}\label{joint-loss}
L_{joint} = \lambda_1 L_{weighted}{(I_g, I_a)} 
+  \lambda_2 L_{weighted}{(I_a', I_a)}, 
\end{equation}

% ----------------------------------------------------------------------------


\subsubsection{Feature Fusion} 
\hspace{10pt} In the method described above, the synthesized image, for bridging the domain gap between the aerial and ground view images,  is only used during the training but is neglected during testing. Since we expect the features of the synthesized image to contain useful information that can help us in retrieval, we attempt to further exploit that information. We fuse the ground image features $f_g$ with synthesized image features $f_a'$ and find a robust representation $f^*_g$ for the query. 
We further train the fused features against the aerial features via fully connected layers that preserves the representative features for query and reference branches, in order to avoid potential pollution of query features during fusion. 

The fusion architecture is shown in Figure \ref{fig:fusion-net}. We first concatenate the features from ground query image with the features from synthesized aerial image. The concatenated features need to be refined to obtain a generalized representation for query image $f^*_g$. We achieve this by passing through a fully-connected layer in the upper branch. 
The lower branch features $f_a$ need to be optimized against the refined features from upper fully-connected layer. So, we add a fully-connected layer in lower branch to obtain a generalized representation of aerial images $f^*_a$. Finally, query feature $f^*_g$ is compared against $f^*_a$ during the testing for image retrieval.
% ----------------------------------------------------------------------------

==> sections/old_method.tex <==
% \clearpage
\section{Method}
We provide an overview of cross-view synthesis GAN, briefly discuss about the loss function used in image retrieval networks and then explain our proposed method \MS{it should not one method, not several method, do not use plural} in this section. 



% ----------------------------------------------------------------------------



% \subsection{Conditional GAN for Cross-View Synthesis} 
% In this work, we synthesize the aerial images from ground-level panorama to use them for image matching. Previous works \cite{Regmi_2018_CVPR, regmi2018cross, Deng:2018:LDG:3274895.3274969, 8490997} have been successful in image translation between aerial and ground-level cropped (single camera) images. Zhai \textit{et al.} \cite{zhai2017crossview} explored the possibility of synthesizing ground-level panorama from aerial images. Here, we transform the query ground level panorama to aerial view. 

% We adopt X-Fork generator architecture  of \cite{Regmi_2018_CVPR} to train the GAN. The X-Fork is a multi-task learning architecture that synthesizes cross-view image as well as semantic segmentation map. Learning to synthesize segmentation map as an auxiliary task greatly helps cross-view synthesis by enforcing the network to preserve the semantic consistency in the target image. 

% The generator of X-Fork has an encoder and two decoders. The network consists of blocks of Convolution, Batch Normalization and Leaky ReLU layers. Convolutional kernels of size 4 x 4 with a stride of 2 are used that downsamples features after each convolution. Since our input is panorama which is of rectangular size, we reshape the features at the bottleneck into square (2 x 2), and then apply multiple upconvolution operations to generate 512 x 512 resolution target image. The six blocks of decoders share the weights whereas the final two blocks don't. One of the branches learns weights to synthesize the target view image while the other branch generates the corresponding semantic map. We first train the GAN to generate the cross-view image $I_a'$ for the ground panorama $I_g$. Next, we use the synthesized images for joint feature learning in our proposed methods.


\subsection{Conditional GAN for Cross-View Synthesis} 

In this work, we synthesize the aerial images from ground-level panorama to use them for image matching. 
Previous works \cite{Regmi_2018_CVPR, regmi2018cross, Deng:2018:LDG:3274895.3274969, 8490997} have been successful in image translation between aerial and ground-level cropped (single camera) images. Zhai \textit{et al.} \cite{zhai2017crossview} explored the possibility of synthesizing ground-level panorama from aerial images. Here, we transform the query ground level panorama to aerial view. 
We adopt X-Fork generator architecture  of \cite{Regmi_2018_CVPR} to train the GAN. 
The X-Fork is a multi-task learning architecture that synthesizes cross-view image as well as semantic segmentation map. Learning to synthesize segmentation map as an auxiliary task greatly helps cross-view synthesis by enforcing the network to preserve the semantic consistency in the target image. 

We make the following modifications to the X-Fork architecture. Since our input is panorama (rectangular in shape), the feature maps at the bottleneck are also rectangular (1x4). 
 We reshape the features into squares (2 x 2), and then apply multiple upconvolution operations to generate 512 x 512 resolution aerial images. Next, we exploit the object edges in input images to provide the network with notion of object shapes and boundaries.  We employ Canny Edge Detection \cite{canny1987computational} to obtain the edgemaps of the inputs.  We stack an edgemap together with the panorama, along the channels to create a 4-channel input; 3 RGB-channels and 1 edgemap channel. 
%  We observe that the 
 The detailed architecture of modified X-Fork network is provided in the supplementary.

% ----------------------------------------------------------------------------



\subsection{Weighted Soft-margin Triplet Loss}

Consider a feature embedding $f_{g}$ for ground-level image, $f_{a-pos}$ for the corresponding matching aerial image and a non-matching aerial image feature $f_{a-neg}$.  The triplet loss \cite{DBLP:journals/corr/HermansBL17} aims to pull the matching feature $f_{a-pos}$ closer to $f_{g}$ while at the same time push $f_{a-neg}$ away. Here, if $d_{p}$ is the Euclidean distance between positive samples ($f_{g}$, $f_{a-pos}$) and $d_{n}$ is the Euclidean distance between negative/non-matching samples ($f_{g}$, $f_{a-neg}$), we try to minimize $d_{p}$ as well as maximize $d_{n}$ using triplet loss. The triplet loss is as shown below:


\vspace{-15pt}
\begin{equation}\label{triplet} 
L_{triplet} = max( 0, m + d_{p} - d_{n}),
\end{equation}

\noindent where, $m$ is a margin that specifies a minimum distance between non-matching pairs. 

In order to avoid the necessity of explicitly deciding the margin for triplet loss, soft-margin triplet loss is popular and is expressed as shown in Equation \ref{triplet-soft}.

\vspace{-15pt}
\begin{equation}\label{triplet-soft}
 L_{soft} = ln( 1 + e^d),
\end{equation}

\noindent where d = $d_{p}$ - $d_{n}$.

We use the weighted soft margin triplet loss\cite{Hu_2018_CVPR} as shown in Equation \ref{weighted-soft}. We use  $ \alpha $ = 10, which  results in better convergence than $ \alpha $ = 1.

\vspace{-15pt}
\begin{equation}\label{weighted-soft}
 L_{weighted} = ln( 1 + e^{\alpha d}).
\end{equation}

 
% ----------------------------------------------------------------------------


\begin{figure}[t]
\begin{center}
  \vspace{-10pt}
   \includegraphics[width=0.98\linewidth]{images/two-stream.pdf}
\end{center}
   \caption{\small Two stream architecture with multi-scale feature aggregation. $\oplus$ represents channelwise concatenation of feature maps.}
\label{fig:two-stream}
   \vspace{-5pt}
\end{figure}
% ----------------------------------------------------------------------------


\subsection{Two Stream Network} 
We employ Siamese-type architecture,  as shown in Figure \ref{fig:two-stream}, where the two encoders do not share the weights. Since the cross-view images are captured from very different viewpoints, entities in one view look different than the entities in the other view. The two branches operate on these sets of diverse images, so it is understandable that the weight sharing is not a good choice. 
Next, we employ multi-scale feature aggregation by preserving the features at three scales. We elegantly exploit the inherent multi-scale pyramidal structure of features at multiple layers of deep neural networks. We consider the features from final three convolutional layers, conv\_6, conv\_7 and conv\_8 layers. These features are aggregated and followed by a fully connected layer to obtain the representation for images in each view. 



Let $X_i$ be a feature map at  \textit{i}$^{th}$ convolutional layer, with feature dimension  $C_i$ x $H_i$ x $W_i$,  where $C_i$, $H_i$ and $W_i$ are channels, height and width respectively. We flatten the feature maps before concatenating them along the channels to obtain the aggregated feature of size: ($C_6$ * $H_6$ * $W_6$) + ($C_7$ * $H_7$ * $W_7$) + ($C_8$ * $H_8$ * $W_8$). Final layer is a fully connected layer that reduces the feature dimensions to 1000. 

We conduct experiments with image pairs of ($I_g$, $I_a$) and ($I_a'$, $I_a$) using two-stream network as baselines in our work. Here, $I_g$ is the ground query image, $I_a$ is the aerial image from reference database and $I_a'$ is the synthesized aerial image generated from $I_g$. We use weighted soft-margin triplet loss shown in Equation \ref{weighted-soft} to learn the feature representations for the image pairs.


% ----------------------------------------------------------------------------

\begin{figure}
\begin{tabular}{c}
\subcaptionbox{Joint Feature Learning: Jointly training on $I_g$ and $I_a'$ through matching them against $I_a$ employing auxiliary loss between $f_a'$ and $f_a$ helps to pull features $f_g$ and $f_a$ closer, and minimize the domain gap between two features when trained using two-stream network shown in Figure \ref{fig:two-stream}.  
\label{fig:aux-loss}} {\includegraphics[width=0.95\linewidth]{images/auxGAN_II.pdf}}\\ \\
\subcaptionbox{Feature Fusion. We fuse the features $f_g$ and $f_a'$ obtained from \ref{fig:aux-loss} and find their common representation $f^*_g$ using fully-connected layer. Similarly, $f_a$ is mapped to $f^*_a$, a domain closer to $f^*_g$. The fully-connected layers are trained, whereas the rest of the network is frozen. \label{fig:fusion-net}} {\includegraphics[width=0.95\linewidth]{images/auxGAN_with_fusion.pdf}}

\end{tabular}
% \vspace{-10pt}
\caption{\small Architectures for our proposed approaches. The green and blue triangles are encoders with the same architecture as encoder branches shown in Figure \ref{fig:two-stream}.}
 \vspace{-10pt}
\end{figure}



% ----------------------------------------------------------------------------


\subsection{Joint Feature Learning and Fusion} 
In this work, we utilize synthesized images constructively as complementary information for the network to exploit during joint feature learning. 
We build upon the generative power of conditional GANs to generate the aerial image for query ground-level panorama. 
Ideally, the synthesized aerial image should be sufficient and capable to retrieve its matching gallery image to justify that cross-view image matching can be solved as cross-view image synthesis followed by the same-view matching. 
% the same-view matching is easier than cross-view matching. 
But, the cross-view synthesis has its own challenges as explained in \cite{Regmi_2018_CVPR} and the synthesized images are noisy; hence cannot be relied upon wholly. Therefore, we attempt to use the synthesized image $I_a'$, as a complementary information during training to bring features $f_g$ and $f_a$ closer by adding an auxiliary loss.  
Next, we fuse the features $f_g$ and $f_a'$ to obtain a joint feature representation $f^*_g$ of query image, and compare it against the aerial feature representation $f^*_a$. 
We combine the features  $f_a'$ and $f_g$ since we expect them to have complementary features, which will be helpful in image retrieval. We provide further explanation below:  


% ----------------------------------------------------------------------------


% \subsubsection{Constructive Learning with Auxiliary Loss} 
\subsubsection{Joint Feature Learning with Auxiliary Loss} 
% \hspace{10pt} In this work, we utilize synthesized images constructively as complementary information for the network to exploit during joint feature learning. 
% We build upon the generative power of conditional GANs to generate the aerial image for query ground-level panorama. 
% Ideally, the synthesized aerial image should be sufficient and capable to retrieve its matching gallery image to justify the same-view matching is easier than cross-view matching. But, the cross-view synthesis has its own challenges as explained in \cite{Regmi_2018_CVPR} and the synthesized images are noisy; hence cannot be relied upon wholly. So, we attempt to use the synthesized image $I_a'$, as a complementary information during training to bring features $f_g$ and $f_a$ closer by adding an auxiliary loss.  
\hspace{10pt} We present a novel approach to leverage the synthesized aerial image in feature learning to assist during cross-view image retrieval.
We employ joint feature learning for real ground query image, ($I_g$), and its transformed version, ($I_a'$). 
The features, $f_g$ for $I_g$ and $f_a'$ for $I_a'$ are jointly optimized against the features $f_a$ for $I_a$. 
The encoder branches for $I_a'$ and $I_a$ share the weights, since both images represent aerial domain. 
This way, the aerial encoder learn weights suitable for the synthesized image $I_a'$ as well as the real image $I_a$. 
Thus, $f_a'$ effectively forces the features $f_a$ to be closer to $f_g$ and bridges the domain gap between the two views. 
This is possible because the transformed image $I_a'$  captures representations of $I_g$ which are easier for the network to learn from $I_a'$ than it would be when comparing $I_a$ directly against $I_g$. 


The network architecture for joint feature learning is shown in Figure \ref{fig:aux-loss}. The encoder blocks are shown in green (for ground image) and blue (for aerial image) triangles. Each encoder consists of the same layers as a branch in Figure \ref{fig:two-stream}. We train our network jointly on these three sets of images ($I_g$, $I_a'$ and $I_a$) using Equation \ref{joint-loss}.  Here, $\lambda_1$ and $\lambda_2$ are balancing factors between the losses for ($I_g$, $I_a$) and ($I_a'$, $I_a$) pairs respectively. During the testing, only the encoders for $I_g$ and $I_a$ are used for feature extraction of real ground and aerial images and retrieval is conducted between the ground image features $f_g$ and aerial image features $f_a$.
% to perform cross-view matching. 

\vspace{-10pt}
\begin{equation}\label{joint-loss}
L_{joint} = \lambda_1 L_{weighted}{(I_g, I_a)} 
+  \lambda_2 L_{weighted}{(I_a', I_a)}, 
\end{equation}

% ----------------------------------------------------------------------------


\subsubsection{Feature Fusion} 
\hspace{10pt} In the method described above, the synthesized image, for bridging the domain gap between the aerial and ground view images,  is only used during the training but is neglected during testing. Since we expect the features of the synthesized image to contain useful information that can help us in retrieval, we attempt to further exploit that information. We fuse the ground image features $f_g$ with synthesized image features $f_a'$ and find a robust representation $f^*_g$ for the query. 
We further train the fused features against the aerial features via fully connected layers that preserves the representative features for query and reference branches, in order to avoid potential pollution of query features during fusion. 

The fusion architecture is shown in Figure \ref{fig:fusion-net}. We first concatenate the features from ground query image with the features from synthesized aerial image. The concatenated features need to be refined to obtain a generalized representation for query image $f^*_g$. We achieve this by passing through a fully-connected layer in the upper branch. 
The lower branch features $f_a$ need to be optimized against the refined features from upper fully-connected layer. So, we add a fully-connected layer in lower branch to obtain a generalized representation of aerial images $f^*_a$. Finally, query feature $f^*_g$ is compared against $f^*_a$ during the testing for image retrieval.
% ----------------------------------------------------------------------------
